Enabling Accelerators for Graph Computing

The advent of Graph Neural Networks (GNNs) has revolutionized the field of machine learning, offering a novel paradigm for learning on graph-structured data. Unlike traditional neural networks, GNNs are capable of capturing complex relationships and dependencies inherent in graph data, making them particularly suited for a wide range of applications including social network analysis, molecular chemistry, and network security. GNNs, with their unique structure and operation, present new computational challenges compared to conventional neural networks. This requires comprehensive benchmarking and a thorough characterization of GNNs to obtain insight into their computational requirements and to identify potential performance bottlenecks. In this thesis, we aim to develop a better understanding of how GNNs interact with the underlying hardware and will leverage this knowledge as we design specialized accelerators and develop new optimizations, leading to more efficient and faster GNN computations. A pivotal component within GNNs is the Sparse General Matrix-Matrix Multiplication (SpGEMM) kernel, known for its computational intensity and irregular memory access patterns. In this thesis, we address the challenges posed by SpGEMM by implementing a highly optimized hashing-based SpGEMM kernel tailored for a custom accelerator. Synthesizing these insights and optimizations, we design state-of-the-art hardware accelerators capable of efficiently handling various GNN workloads. Our accelerator architectures are built on our characterization of GNN computational demands, providing clear motivation for our approaches. This exploration into novel models underlines our comprehensive approach, as we strive to enable accelerators that are not just performant, but also versatile, able to adapt to the evolving landscape of graph computing.

==> tables/arch_implications.tex <==

% \begin{table}[tb]
% \centering
% \caption{Architectural implications of GNN Models}
% \vspace*{-2mm}
% \label{tab:arch_impl}
% \resizebox{\columnwidth}{!}{%
% \begin{tabular}{c | l } 
%     % \hline
%     % \hline
%     \toprule[1pt]
%    \textbf{Model} & Features requiring architectural support \\
%     \hline
%     \hline

%     \multirow{2}{*}{GCN}~\cite{kipf2016semi} &  $\bullet$ Requires efficient memory management for large-scale graphs  \\
%       &  $\bullet$ Requires effective load balancing for graphs with varying degrees \\
%     \hline
%     \multirow{2}{*}{GIN}~\cite{xu2018powerful} &  $\bullet$ Requires \textit{edge-embedding} support \\
%         &  $\bullet$ Requires MLP-aggregators for node transformations \\
%     \hline
%     \multirow{2}{*}{GAT}~\cite{velivckovic2017graph} & $\bullet$ Requires dynamically updated $\alpha$ activation \\
%        & $\bullet$ Requires \textit{anisotropic} aggregators  \\    
%     % \hline
%     \hline
%     \multirow{2}{*}{SAGE}~\cite{hamilton2017inductive} & $\bullet$ Requires \textit{ReLU} and \textit{max} activation functions \\
%        & $\bullet$ Requires \textit{max-pool} and \textit{LSTM} aggregators \\
    
%     \hline
%     PNA~\cite{corso2020principal} & $\bullet$ Requires \textit{min}, \textit{max}, \textit{sum}, \textit{mean}, and \textit{std-dev} aggregators \\
%      & $\bullet$ Requires support for \textit{degree-scaling method} \\
%     \hline
%     DGN~\cite{beaini2021directional} & $\bullet$ Requires support for directional aggregation matrix  \\
    
%     \bottomrule[1pt]

% \end{tabular}%
% }

% % \scriptsize

% % \centering
% % $^{*}$ Hello 

% \vspace*{-6mm}

% \end{table}

==> tables/datasets.tex <==
% \begin{table*}[ht]
% \centering
% \caption{GNN Workloads Supported by NeuraChip}
% \vspace*{-2mm}
% \begin{tabularx}{\textwidth}{@{}l>{\RaggedRight}p{3.0cm}>{\RaggedRight}p{3.0cm}>{\RaggedRight}p{3.0cm}>{\RaggedRight}p{3.6cm}rr@{}}
%   \toprule
%   \thead{Abbv} & \thead{GNN Model} & \thead{Application Domain} & \thead{Graph Input Type} & \thead{Datasets} & \thead{\# Node} & \thead{\# Edge} \\
%   \midrule
%   \multirow{2}{*}{\textbf{GCN}} & 
%   \multirow{2}{=}{Graph Convolutional Networks} & 
%   \multirow{2}{=}{Recommendation Systems} & 
%   \multirow{2}{=}{Homogeneous Graph} & 
      
%       Nowplaying~(NWP) \cite{zangerle2014nowplaying} & 22.9M & 1.9M \\
      
%       \arrayrulecolor{black!10}\cmidrule{5-7}
      
%       &&&&
%       Movielens~(MVL)~\cite{harper2015movielens} & 1.9M & 9.7K 
%       \\
     
%   \arrayrulecolor{black!20}\midrule
      
%   \multirow{2}{*}{\textbf{GIN}} & 
%   \multirow{2}{=}{Graph Isomorphism Network} & 
%   \multirow{2}{=}{Computational Chemistry} & 
%   \multirow{2}{=}{Homogeneous Graph} & 
      
%       LA  \cite{yu2018spatio} \todo{cant find this work} & 207 & 325  \\
      
%       \arrayrulecolor{black!10}\cmidrule{5-7}
      
%       &&&&
%       PEMS\_Bay~(PEMS) \cite{yu2018spatio} & 1722 & 2694\\
      
      
%     \arrayrulecolor{black!20}\midrule
      
%   \multirow{2}{*}{\textbf{GAT}} & 
%   \multirow{2}{=}{Graph Attention Network} & 
%   \multirow{2}{=}{Traffic Forecasting} & 
%   \multirow{2}{=}{Heterogenous Graph} & 
%       MOLHIV  \cite{hu2020open} & 1.04M & 1.1M \\
%       \arrayrulecolor{black!10}\cmidrule{5-7}
%      &&&&
%       MOLTOX  \cite{hu2020open} & 145K & 151K \\
      
      
%   \arrayrulecolor{black!20}\midrule
  
%   \multirow{2}{*}{\textbf{SAGE}} & 
%   \multirow{2}{=}{Graph Sample and AggregatE} & 
%   \multirow{2}{=}{Online Social Networks} & 
%   \multirow{2}{=}{Dynamic Graph} & 
%       MOLHIV  \cite{hu2020open} & 1.04M & 1.1M \\
%       \arrayrulecolor{black!10}\cmidrule{5-7}
%      &&&&
%       MOLTOX  \cite{hu2020open} & 145K & 151K \\
 
%   \arrayrulecolor{black!20}\midrule
  
%   \multirow{2}{*}{\textbf{PNA}} & 
%   \multirow{2}{=}{Principled Neighbor Aggregation} & 
%   \multirow{2}{=}{Predicting Molecular Properties} & 
%   \multirow{2}{=}{Homogeneous Graph} & 
%       MOLHIV  \cite{hu2020open} & 1.04M & 1.1M \\
%       \arrayrulecolor{black!10}\cmidrule{5-7}
%      &&&&
%       MOLTOX  \cite{hu2020open} & 145K & 151K \\
%   \arrayrulecolor{black!20}\midrule
  
  
%   \multirow{4}{*}{\textbf{DGN}} & 
%   \multirow{4}{=}{Directional Graph Networks} & 
%   \multirow{4}{=}{Computational Biology} & 
%   \multirow{4}{=}{Homogeneous Graph} & 
%     Cora \cite{yang2016revisiting} & 2K & 10.5K  \\
%       \arrayrulecolor{black!10}\cmidrule{5-7}
%       &&&&
%       CiteSeer~(CSEER) \cite{yang2016revisiting} & 3.3K & 9.2K\\
%       \arrayrulecolor{black!10}\cmidrule{5-7}
%       &&&&
%       PubMed~(CSEER) \cite{yang2016revisiting} & 19.7K & 88.6K\\
%       \arrayrulecolor{black!10}\cmidrule{5-7}
%       &&&&
%       Protein-Interaction~(PPI) \cite{yang2016revisiting} & 19.7K & 88.6K\\
%   %     \arrayrulecolor{black!20}\midrule
  
%   % \multirow{1}{*}{\textbf{TLSTM}} & 
%   % \multirow{1}{=}{Tree Long Short-Term Memory Networks} & 
%   % \multirow{1}{=}{Sentiment Classification} & 
%   % \multirow{1}{=}{Homogeneous Graph} & 
%   %     Stanford Sentiment Treebank~(SNTM)~\cite{socher2013recursive}  & 318K & 310K  \\

%   \arrayrulecolor{black}\bottomrule
% \end{tabularx}

% \label{tab:benchmarks}
% \vspace{-0.5cm}
% \end{table*}





% \begin{table}
% \centering
% \caption{Properties of graph datasets used for evaluating NeuraChip across six different GNN workloads.}
% \vspace*{-2mm}
% \label{tab:datasets}
% \begin{tabular}{p{0.62in} | x{0.33in} x{0.33in} x{0.5in} x{0.38in} x{0.4in}}
% \arrayrulecolor{black}\toprule
%     \textbf{Datasets}& \textbf{Graph Count} &  \textbf{Node Count} & \textbf{Edge Count} & \textbf{Density} & \textbf{Avg. Degree} \\ [0.5ex] 
% \arrayrulecolor{black}\toprule
% \arrayrulecolor{black}\toprule
%     Cora~\cite{yang2016revisiting} & $1$ & $2,708$ & $13,264$ & $1.8e-3$ & $4.9$ \\
%     \arrayrulecolor{black!20}\midrule
%     CiteSeer~\cite{yang2016revisiting} & $1$ &  $3,327$ & $12,431$ & $1.1e-3$ & $3.74$ \\
%     \arrayrulecolor{black!20}\midrule
%     PubMed~\cite{yang2016revisiting} & $1$ &  $19717$ & $108,365$ & $2.8e-4$ & $5.5$ \\
%     \arrayrulecolor{black!20}\midrule
%     US-Airports~\cite{ribeiro2017struc2vec} & $1$ &  $1,190$ & $13,599$ & $9.6e-3$ & $11.4$ \\
%     \arrayrulecolor{black!20}\midrule
%     Reddit~\cite{kumar2019predicting} & $1$ &  $2.3e5$ & $1.1e8$ & $2.1e-3$ & $493$ \\
%     \arrayrulecolor{black!20}\midrule
%     Amazon~\cite{shchur2018pitfalls} & $1$ &  $2.4e6$ & $1.2e8$ & $2.1e-5$ & $51.5$ \\
%     \arrayrulecolor{black!20}\midrule
%     MolHIV~\cite{hu2020open} & $4113$ &  $25.3$ & $55.6$ & $8.6e-2$ & $2.2$ \\
%     \arrayrulecolor{black!20}\midrule
%     MolPCBA~\cite{hu2020open} & $43773$ &  $27.0$ & $59.3$ & $8.1e-2$ & $2.2$ \\
    

%      \arrayrulecolor{black}\bottomrule
% % \vspace{-2.7em}
% \end{tabular}
% \vspace{-8mm}
% \end{table}


==> tables/dram_config.tex <==

\begin{table}
\centering
\caption{DRAMsim3 HBM2 configuration}
% \vspace*{2mm}
\label{tab:hbm_config}

\begin{tabular}{l | c } 
    % \hline
    % \hline
    \toprule[1pt]
   \textbf{Parameter} & Value \\
    \arrayrulecolor{black}\toprule
    \arrayrulecolor{black}\toprule
    % \\[-1.5ex]
    Number of stacks & $1$-\texttt{hi} \\
    \arrayrulecolor{black!20}\midrule
    Total Size & $8$ \texttt{GB} \\
    \arrayrulecolor{black!20}\midrule
    Dies per stack & $8$ \\
    \arrayrulecolor{black!20}\midrule
    Total channels & $8$ \\
    \arrayrulecolor{black!20}\midrule
    Bank groups & $4$ \\
    \arrayrulecolor{black!20}\midrule
    Banks per group & $4$ \\
    \arrayrulecolor{black!20}\midrule
    Bus width & $128$ bit wide \\
    \arrayrulecolor{black!20}\midrule
    Burst Length (BL) & $4$ \\
    \arrayrulecolor{black!20}\midrule
    Peak pin bandwidth & $2$ \texttt{GT/s} \\
    \arrayrulecolor{black!20}\midrule
    Peak channel bandwidth & $32$ \texttt{GB/s} \\
    \arrayrulecolor{black}\bottomrule

    \textbf{Peak memory bandwidth} & \textbf{$256$ \texttt{GB/s}} \\
    
    
   
    % \hline
    \arrayrulecolor{black}\bottomrule

\end{tabular}



\end{table}

==> tables/gnn_equations.tex <==
\begin{table}
\centering
\caption{Supported GNN workloads by NeuraChip's native hash engines}
% \vspace*{2mm}
\label{tab:gnn_equations}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{l | c c } 
    % \hline
    % \hline
    \toprule[1pt]
   \textbf{Model} & Model Formulation & x \\
    \hline
    \hline
    % \\[-1.5ex]
   GCN & $H^{(l+1)} = \sigma\left(\tilde{D}^{-\frac{1}{2}}\tilde{A}\tilde{D}^{-\frac{1}{2}}H^{(l)}W^{(l)}\right)$ & b\\
   GIN & $h^{(l+1)}_{v} = \sigma\left((1 + \epsilon^{(l)})h^{(l)}_{v} + \sum_{u \in \mathcal{N}(v)} W^{(l)}h^{(l)}_{u}\right)$ & b\\
   SAGE & $h_v^{(l)} = \sigma\left(W_l \cdot \text{CONCAT}\left(h_v^{(l-1)}, h_{N_s(v)}^{(l)}\right)\right)$ & b\\
   GAT & $h_i^{(l+1)} = \sigma \left( \sum_{j \in \mathcal{N}(i)} \alpha_{ij}^{(l)} W^{(l)} h_j^{(l)} \right)$ & b\\
   PNA & $h_v^{(l+1)} = \sigma\left(W^{(l)}h_v^{(l)} + \sum_{\text{deg}(v)=k} \frac{1}{|\mathcal{V}_k|} \sum_{v' \in \mathcal{V}_k} \phi(\mathcal{N}(v'))\right)$ & b\\
   DGN & x & b\\
   
    % \hline
    \bottomrule[1pt]

\end{tabular}%
}

\scriptsize

\centering
$^{*}$ Hello


\end{table}

==> tables/isa.tex <==
\begin{table}[htbp]
\centering
\caption{NeuraChip extended  MicroISA}
% \vspace*{2mm}
\label{tab:isa}
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{l| p{2.0in} } 
    % \hline
    % \hline
    \toprule[1pt]
   \textbf{Instruction} & Description \\
\arrayrulecolor{black}\toprule
\arrayrulecolor{black}\toprule
    \texttt{hash\_insert} & Insert hash entry into HashPad \\
    \arrayrulecolor{black!20}\midrule
    \texttt{hash\_update} & Update an existing hash entry in HashPad \\
    \arrayrulecolor{black!20}\midrule
    \texttt{hash\_accumulate} & Insert or update hash entry while accumulating the previous entry \\
    % \arrayrulecolor{black!20}\midrule
    % \texttt{hash\_invalidate} & Evict the hash line and write back to main memory \\
    % \arrayrulecolor{black!20}\midrule
    % \texttt{hash\_broadcast} & Accumulate a single element onto multiple hash lines \\
    % \arrayrulecolor{black!20}\midrule
    % \texttt{hash\_scatter} & Accumulate a multiple elements onto multiple hash lines \\
    % \arrayrulecolor{black!20}\midrule
    % \texttt{hash\_reduce} & Coalesce multiple hash instructions before hashing onto HashPad \\
    
    
    \arrayrulecolor{black}\bottomrule
% \vspace{-1.0em}
\end{tabular}%
% }

% \scriptsize

% \centering
% $^{*}$ Hello 


% \vspace{-1.7em}

\end{table}

==> tables/latency_table.tex <==



% \begin{table}
% \centering
% \caption{Percentage Speedup of NeuraChip Tile-$16$ over SOTA accelerators. Latency values are in $\mu$s.}
% % \vspace*{2mm}
% \label{tab:latency_compare}
% \resizebox{1\linewidth}{!}{%
% \begin{tabular}{p{0.3in} | x{0.1in} x{0.1in} x{0.1in} x{0.1in} x{0.1in} x{0.1in} x{0.1in} x{0.1in} | x{0.1in} x{0.1in} x{0.1in} x{0.1in} x{0.1in}} 
%     % \hline
%     % \hline
%     % \toprule[1pt]
%    \textbf{Models} & \rotatebox{90}{Cora} & \rotatebox{90}{CiteSeer} & \rotatebox{90}{PubMed} & \rotatebox{90}{US-Airports} & \rotatebox{90}{Reddit (ms)} & \rotatebox{90}{Amazon (ms)} & \rotatebox{90}{MolHIV} & \rotatebox{90}{MolPCBA} & \rotatebox{90}{I-GCN~\cite{geng2021gcn}} & \rotatebox{90}{AWB-GCN~\cite{geng2021gcn}} & \rotatebox{90}{HyGCN~\cite{geng2021gcn}} & \rotatebox{90}{GROW~\cite{geng2021gcn}} & \rotatebox{90}{FlowGNN~\cite{geng2021gcn}}\\
%     \arrayrulecolor{black}\toprule
%     \arrayrulecolor{black}\toprule
%     % \\[-1.5ex] GAT$1.9$ & PNA$2.6$ & DGN$1.7$ 
%    GCN & $1.8$ & $2.2$ & $13.6$ & $1.9$ & $24$ & $25$ & $5.5$ & $5.5$ & $16.6$ & $22.4$ & $8.1$ & $14.6$ & $18.8$ \\
%    \arrayrulecolor{black!20}\midrule
%    GIN & $2.4$ & $2.9$ & $17.9$ & $2.6$ & $33$ & $36$ & $5.1$ & $5.1$ & $21.8$ & \cross & $19.6$ & $11.7$ & $17.6$ \\
%    \arrayrulecolor{black!20}\midrule
%    GAT & $1.9$ & $2.3$ & $12.6$ & $1.9$ & $26$ & $31$ & $3.6$ & $3.7$ & \cross & \cross & \cross & $6.4$ & $2.3$ \\
%    \arrayrulecolor{black!20}\midrule
%    SAGE & $2.7$ & $3.1$ & $16.6$ & $2.9$ & $36$ & $37$ & $5.0$ & $5.1$ & $20.4$ & \cross & $19.1$ & $9.5$ & $17.2$ \\
%    \arrayrulecolor{black!20}\midrule
%    PNA & $2.6$ & $3.3$ & $17.6$ & $2.9$ & $34$ & $35$ & $9.4$ & $9.8$ & \cross & \cross & \cross & \cross & $6.3$ \\
%    \arrayrulecolor{black!20}\midrule
%    DGN & $1.7$ & $2.1$ & $13.1$ & $1.9$ & $23$ & $21$ & $15.9$ & $16.7$ & \cross & \cross & \cross & \cross & $4.7$ \\
   

%     % \hline
%     \arrayrulecolor{black}\bottomrule

% \end{tabular}
% }% adjustbox


% % \scriptsize

% % \centering
% % $^{*}$ Hello

% \end{table}




\begin{table}
\centering
\caption{Percentage Speedup of NeuraChip over prior GNN accelerators.}
% \vspace*{2mm}
\label{tab:latency_compare}
\resizebox{1\linewidth}{!}{%
\begin{tabular}{p{0.35in} | x{0.1in} x{0.1in} x{0.1in} x{0.1in} x{0.1in} x{0.1in} | x{0.1in} x{0.1in} x{0.1in} x{0.1in} x{0.1in}} 
    % \hline
    % \hline
    % \toprule[1pt]
   \rotatebox{90}{\textbf{Tile Config}} & \rotatebox{90}{Cora ($\mu$s)} & \rotatebox{90}{CiteSeer ($\mu$s)} & \rotatebox{90}{PubMed ($\mu$s)} & \rotatebox{90}{US-Airports ($\mu$s)} & \rotatebox{90}{Reddit (ms)} & \rotatebox{90}{Amazon (ms)} & \rotatebox{90}{I-GCN~\cite{geng2021gcn}} & \rotatebox{90}{AWB-GCN~\cite{geng2020awb}} & \rotatebox{90}{HyGCN~\cite{yan2020hygcn}} & \rotatebox{90}{GROW~\cite{hwang2023grow}} & \rotatebox{90}{FlowGNN~\cite{sarkar2023flowgnn}}\\
    \arrayrulecolor{black}\toprule
    \arrayrulecolor{black}\toprule
    % \\[-1.5ex] GAT$1.9$ & PNA$2.6$ & DGN$1.7$ 
   Tile-4 & $1.8$ & $2.2$ & $13.6$ & $1.9$ & $24$ & $25$ & $16.6$ & $22.4$ & $8.1$ & $14.6$ & $18.8$ \\
   \arrayrulecolor{black!20}\midrule
   Tile-16 & $2.4$ & $2.9$ & $17.9$ & $2.6$ & $33$ & $36$ & $21.8$ & \cross & $19.6$ & $11.7$ & $17.6$ \\
   \arrayrulecolor{black!20}\midrule
   Tile-64 & $1.9$ & $2.3$ & $12.6$ & $1.9$ & $26$ & $31$ & \cross & \cross & \cross & $6.4$ & $2.3$ \\
   % \arrayrulecolor{black!20}\midrule
   % SAGE & $2.7$ & $3.1$ & $16.6$ & $2.9$ & $36$ & $37$ & $5.0$ & $5.1$ & $20.4$ & \cross & $19.1$ & $9.5$ & $17.2$ \\
   % \arrayrulecolor{black!20}\midrule
   % PNA & $2.6$ & $3.3$ & $17.6$ & $2.9$ & $34$ & $35$ & $9.4$ & $9.8$ & \cross & \cross & \cross & \cross & $6.3$ \\
   % \arrayrulecolor{black!20}\midrule
   % DGN & $1.7$ & $2.1$ & $13.1$ & $1.9$ & $23$ & $21$ & $15.9$ & $16.7$ & \cross & \cross & \cross & \cross & $4.7$ \\
   

    % \hline
    \arrayrulecolor{black}\bottomrule

\end{tabular}
}% adjustbox


% \scriptsize

% \centering
% $^{*}$ Hello



\end{table}

==> tables/prior_compare.tex <==



\begin{table*}
\centering
\caption{Comparative analysis of the GNN model compatibility and features of NeuraChip accelerator, relative to SOTA accelerators}
\vspace*{-2mm}
\label{tab:prior_compare}

\begin{tabular}{l | c c c c c c | x{0.34in} x{0.7in} x{0.37in} x{0.5in} x{0.5in} x{0.33in} } 
    % \hline
    % \hline
    % \toprule[1pt]
    \arrayrulecolor{black}\toprule
   \textbf{Accelerator} & GCN & GIN & GAT & SAGE & PNA & DGN & Kernel Fusion & Loop Reordering & Pruning & Bank Mapping & Load Balancing & Hash-based \\
   \arrayrulecolor{black}\toprule
   \arrayrulecolor{black}\toprule
   % \arrayrulecolor{black!20}\bottomrule
    % \\[-1.5ex]
   I-GCN~\cite{geng2021gcn} & \tick & \tick & \cross & \tick & \cross & \cross & \cross & \cross & \tick & \tick & \tick  & \cross \\
   \arrayrulecolor{black!20}\midrule
   AWB-GCN~\cite{geng2020awb} & \tick & \cross & \cross & \cross & \cross & \cross & \tick & \tick & \cross & \tick & \tick & \cross \\
   \arrayrulecolor{black!20}\midrule
   HyGCN~\cite{yan2020hygcn} & \tick & \tick & \cross & \tick & \cross & \cross & \tick & \tick & \cross & \tick & \tick & \cross \\
   \arrayrulecolor{black!20}\midrule
   EnGN~\cite{liang2020engn} & \tick & \cross & \cross & \tick & \cross & \cross & \cross & \tick & \cross & \tick & \tick & \cross \\
   \arrayrulecolor{black!20}\midrule
   GraphPE~\cite{auten2020hardware} & \tick & \cross & \tick & \cross & \cross & \cross & \cross & \cross & \cross & \tick & \cross & \cross \\
   \arrayrulecolor{black!20}\midrule
   GNNerator~\cite{stevens2021gnnerator} & \tick & \cross & \cross & \tick & \cross & \cross & \cross & \cross & \cross & \cross & \cross & \cross \\
   \arrayrulecolor{black!20}\midrule
   GCoD~\cite{you2022gcod} & \tick & \tick & \tick & \tick & \cross & \cross & \cross & \tick & \tick & \cross & \tick & \cross \\
   \arrayrulecolor{black!20}\midrule
   ReGNN~\cite{chen2022regnn} & \tick & \tick & \cross & \tick & \cross & \cross & \tick & \cross & \cross & \cross & \tick & \cross \\
   \arrayrulecolor{black!20}\midrule
   ReFlip~\cite{huang2022accelerating} & \tick & \tick & \tick & \tick & \cross & \cross & \cross & \cross & \cross & \cross & \tick & \cross \\
   \arrayrulecolor{black!20}\midrule
   GROW~\cite{hwang2023grow} & \tick & \tick & \tick & \tick & \cross & \cross & \cross & \tick & \cross & \cross & \tick & \cross \\
   \arrayrulecolor{black!20}\midrule
   FlowGNN~\cite{sarkar2023flowgnn} & \tick & \tick & \tick & \tick & \tick & \tick & \tick & \cross & \cross & \tick & \tick & \cross \\
   \arrayrulecolor{black!20}\midrule
   % \arrayrulecolor{black}\bottomrule
   \textbf{NeuraChip} & \tick & \tick & \tick & \tick & \tick & \tick & \tick & \tick & \tick & \tick & \tick & \tick \\
    % \hline
   \arrayrulecolor{black}\bottomrule

\end{tabular}


% \scriptsize

% \centering

% \diamd \  \todo{Address diamonds}

\vspace*{-6mm}

\end{table*}


==> tables/spgemm_compare.tex <==



\begin{table*}
\centering
\caption{Performance comparison of state-of-the-art SpGEMM accelerators across various NeuraChip system configurations.}

\label{tab:spgemm_compare}

\begin{tabular}{x{0.90in} | x{0.40in} x{0.47in} x{0.40in} x{0.40in} x{0.61in} x{0.45in} x{0.53in} x{0.53in} x{0.53in} } 
    % \hline
    % \hline
    % \toprule[1pt]
    \arrayrulecolor{black}\toprule
   \textbf{Architectural Parameters} & Xeon E5 & NVIDIA H100 & AMD MI100 & Outer SPACE & SpArch & Gamma & \textbf{NeuraChip Tile-4} & \textbf{NeuraChip Tile-16} & \textbf{NeuraChip Tile-64} \\
   \arrayrulecolor{black}\toprule
   \arrayrulecolor{black}\toprule
   Compute Units & 8 Cores AVX2 & 7296 FP64 & 7680 FP64 & $256$~PEs & $2\times8$~Mults $16~\times~16$~Merger  & $32$~PEs Radix-$64$ & $2\times4$ NeuraCores & $2\times16$ NeuraCores & $2\times64$ NeuraCores \\
   \arrayrulecolor{black!20}\midrule
   Frequency $(\mathrm{GHz})$ & $2.9$ & $1.6$ & $1.5$ & $1.5$ & $1$ & $1$ & $1$ & $1$ & $1$ \\
   \arrayrulecolor{black!20}\midrule
   Peak Performance & $186$ $\mathrm{GFLOPs}$ & $26$ $\mathrm{TFLOPs}$ & $11.5$ $\mathrm{TFLOPs}$ & $384$ $\mathrm{GFLOPs}$ & $32$ $\mathrm{GFLOPs}$ & $32$ $\mathrm{GFLOPs}$ & $8$ $\mathrm{GFLOPs}$ & $32$ $\mathrm{GFLOPs}$ & $128$ $\mathrm{GFLOPs}$ \\
   \arrayrulecolor{black!20}\midrule
   SpGEMM Perf.$^{\Phi}$ $(\mathrm{GOP}/s)$ & $1.12$ & $1.86$ & $1.48$ & $2.9$ & $10.4$ & $16.5$ & $5.15$ & $24.75$ & $30.69$ $93.17^{\alpha}$  \\
   \arrayrulecolor{black!20}\midrule
   On-chip Memory & $15~\mathrm{MB}^{\tau}$ & $50~\mathrm{MB}^{\dagger}$ & $8~\mathrm{MB}^{\dagger}$ & $4~\mathrm{MB}$ & $15~\mathrm{MB}^{\star}$ & $3~\mathrm{MB}^{\ast}$ & $0.75~\mathrm{MB}^{\delta}$ & $3~\mathrm{MB}^{\delta}$ & $12~\mathrm{MB}^{\delta}$ \\
   \arrayrulecolor{black!20}\midrule
   Off-chip Memory & DDR4 $136\mathrm{GB}/\mathrm{s}$ & HBM $2\mathrm{TB}/\mathrm{s}$ & HBM $1.2\mathrm{TB}/\mathrm{s}$ & HBM $128\mathrm{GB}/\mathrm{s}$ & HBM $128\mathrm{GB}/\mathrm{s}$ & HBM $128\mathrm{GB}/\mathrm{s}$ & HBM $128\mathrm{GB}/\mathrm{s}$ & HBM $128\mathrm{GB}/\mathrm{s}$ & HBM $128\mathrm{GB}/\mathrm{s}$ \\
   \arrayrulecolor{black!20}\midrule
   Technology $(nm)$ & $32$ & $4$ & $7$ & $32$ & $40$ & $45$ & $7$ & $7$ & $7$ \\
   \arrayrulecolor{black!20}\midrule
   Area $(mm^2)$ & $356$ & $814$ & $750$ & $86.74$ & $28.49$ & $30.6^{\ddagger}$ $20.44^{\ddagger}$ & $2.37$ & $10.2$ & $35.26$ \\
   \arrayrulecolor{black!20}\midrule
   Power $(W)$ & $85^{\diamond}$ & $300^{\diamond}$ & $300^{\diamond}$ & $24$ & $9.26$ & \ding{118} & $11.46$ & $16.06$ & $24.22$ \\
   \arrayrulecolor{black!20}\midrule
   Energy Efficiency $(\mathrm{GOPS}/W)$ & \ding{117} & \ding{117} & \ding{117} & $0.120$ & $1.123$ & \ding{118} & $0.449$ & $1.541$ & $1.266$ \\
   \arrayrulecolor{black!20}\midrule
   Area Efficiency $(\mathrm{GOPS}/mm^2)$ & \ding{117} & \ding{117} & \ding{117} & $0.034$ & $0.365$ & $0.539$ & $2.171$ & $2.426$ & $0.870$ \\
   \arrayrulecolor{black!20}\midrule
   Tile-16 Speedup & $22.1\times$ & $13.3\times$ & $16.7\times$ & $6.6\times$ & $2.4\times$ & $1.5\times$ & $4.8\times$ & $1\times$ & $0.807\times$ \\
   \arrayrulecolor{black}\bottomrule

\end{tabular}

\vspace*{0.5mm}

\scriptsize

% \centering

$\diamond$Max thermal dissipation power from datasheet
\ding{118}Gamma does not provide a power performance model
$^{\dagger}$ L2 cache size
$^{\tau}$ L3 cache size
$^{\delta}$HashPad Size
$^{\ast}$FiberCache Size

\ding{117}Power and area metrics were sourced from the vendor's datasheets, thus derived metrics have not been included.
$^{\alpha}$ Simulated using dual stacked HBM providing peak bandwidth of $256$ GB/s
${\ddagger}$Gamma synthesizes accelerator using both $45$ nm and $40$ nm processes, resulting in computing areas of $30.6$ $mm^2$ and $20.44$ $mm^2$, respectively




$^{\star}$Represents column fetchers, row prefetchers, and partial matrix fetchers and writers.
$^{\Phi}$Computed on common set of matrices as shown in Table I.

\end{table*}

